Sample Elicitation

It is important to collect credible training samples $(x,y)$ for building data-intensive learning systems (e.g., a deep learning system). Asking people to report complex distribution $p(x)$, though theoretically viable, is challenging in practice. This is primarily due to the cognitive loads required for human agents to form the report of this highly complicated information. While classical elicitation mechanisms apply to eliciting a complex and generative (and continuous) distribution $p(x)$, we are interested in eliciting samples $x_i \sim p(x)$ from agents directly. We coin the above problem "sample elicitation". This paper introduces a deep learning aided method to incentivize credible sample contributions from self-interested and rational agents. We show that with an accurate estimation of a certain $f$-divergence function we can achieve approximate incentive compatibility in eliciting truthful samples. We then present an efficient estimator with theoretical guarantees via studying the variational forms of the $f$-divergence function. We also show a connection between this sample elicitation problem and $f$-GAN, and how this connection can help reconstruct an estimator of the distribution based on collected samples. Experiments on synthetic data, MNIST, and CIFAR-10 datasets demonstrate that our mechanism elicits truthful samples. Our implementation is available at https://github.com/weijiaheng/Credible-sample-elicitation.git.

==> estimation.tex <==
%!TEX root =pp-sample.tex

\section{Estimation of $f$-divergence}\label{section:subproblem_fdiv}
In this section, we introduce an estimator of $f$-divergence and establish the statistical rate of convergence, which characterizes $\epsilon(n)$ and $\delta(n)$. 
 For the simplicity of presentation, in the sequel, we estimate the $f$-divergence $D_f(q\|p)$ between  distributions $\PP$ and $\QQ$ with probability density functions $p$ and $q$, respectively.  The rate of convergence of the estimated $f$-divergence can be easily extended to that of the estimated mutual information.  


Following from the analysis in Section \ref{eq:sec-se}, by Fenchel duality,  estimating $f$-divergence between $\PP$ and $\QQ$ is equivalent to solving the following optimization problem, 
\#\label{eq:subproblem_popu}
&t^*(\cdot;p,q) = \argmin_{t(\cdot)} \EE_{x\sim \PP}[ f^\dagger(t(x))] - \EE_{x\sim \QQ}[t(x)] ,\notag\\
&D_f(q\|p) =  \EE_{x\sim\QQ}[  t^*(x;p,q) ] -\EE_{x\sim\PP}[ f^\dagger( t^*(x;p,q) )].
\#
A natural way to estimate the divergence $D_f(q\| p)$ is to solve the empirical counterpart of \eqref{eq:subproblem_popu} as follows, 
\#\label{eq:gen-form}
&t^\natural(\cdot;p,q) = \argmin_{t\in\Phi} \EE_{x\sim\PP_n}[ f^\dagger(t(x))] - \EE_{x\sim\QQ_n}[t(x)] ,\notag\\
& D_f^\natural (q\|p) =  \EE_{x\sim\QQ_n}[ t^\natural(x;p,q) ] -\EE_{x\sim\PP_n}[ f^\dagger( t^\natural(x;p,q) )], 
\#
where $\Phi$ is a function space with functions whose infinity norm is bounded by some constant $M$. 

To establish the statistical rate of convergence for such an estimator in \eqref{eq:gen-form}, we introduce the following definition of covering number. 

\begin{definition}[Covering Number]
Let $(V, \|\cdot \|_{L_2})$ be a normed space, and $\Phi \subset V$. We say that $\{v_1, \ldots, v_N\}$ is a $\delta$-covering over $\Phi$ of size $N$ if $\Phi\subset\cup_{i = 1}^N B(v_i, \delta)$, where $B(v_i, \delta)$ is the $\delta$-ball centered at $v_i$.  The covering number is defined as $N_2(\delta, \Phi) = \min\{ N\colon  \exists \delta\textrm{-covering over $\Phi$ of size $N$} \}$. 
\end{definition}

We impose the following assumption on the covering number of the space $\Phi$, which characterizes the representation power of  $\Phi$. 

\begin{assumption}\label{assum:phi-cn}
We have $N_2(\delta, \Phi) = \cO( \exp\{ \delta^{-\gamma_\Phi} \})$, where $0 < \gamma_\Phi < 2$. 
\end{assumption}

In the following theorem, we establish the statistical convergence rate of the estimator proposed in \eqref{eq:gen-form}. For the simplicity of discussion, we assume that $t^* \in \Phi$. 

\begin{theorem}\label{thm:gen}
Suppose that Assumptions \ref{assum:ratio}, \ref{assumption:reg}, and \ref{assum:phi-cn} hold, and $t^*(\cdot; p, q)\in \Phi$. With probability at least $1- \exp(-n^{\gamma_\Phi / (2 + \gamma_\Phi)} )$, we have
\$
| D_f^\natural(q\| p) - D_f(q\| p)| \lesssim n^{-1/(\gamma_\Phi + 2)}. 
\$
\end{theorem}

We defer the proof of Theorem \ref{thm:gen} to Section \S\ref{proof:thm:gen}.  By Theorem \ref{thm:gen}, the estimator in \eqref{eq:gen-form} achieves the optimal nonparametric rate of convergence \citep{stone1982optimal}. 



\subsection{Estimation via Deep Neural Networks}\label{sec:est-dnn}

Since the most general estimator $D_f^\natural (q\|p)$ proposed in \eqref{eq:gen-form} requires solving an optimization problem over a function space, which is usually intractable, we introduce an estimator of the $f$-divergence $D_f(q\| p)$ using the family of deep neural networks in this section.    We now define the family of deep neural networks as follows. 

\begin{definition}\label{def:nn_set}
Given a vector $k = (k_0, \ldots, k_{L+1})\in\NN^{L+2}$, where $k_0 = d$ and $k_{L+1} = 1$, the family of deep neural networks is defined as
\$
\Phi(L, k) = \{ & \varphi(x; W, v) = W_{L+1}\sigma_{v_L}\cdots W_{2}\sigma_{ v_1}W_1 x\colon \notag\\
&\qquad   W_{j}\in\RR^{k_j\times k_{j-1}}, v_{j}\in\RR^{k_j} \}. 
\$
where $\sigma_{v}(x) = \max\{0, x-v\}$ is the ReLU activation function. 
\end{definition}

To avoid overfitting, the sparsity of the deep neural networks is a typical assumption  in  deep learning literature.   In practice, such a sparsity property is achieved through certain techniques, e.g., dropout \citep{srivastava2014dropout},  or certain network architecture, e.g., convolutional neural network \citep{krizhevsky2012imagenet}.  We now define the family of sparse neural networks as follows, 
\#\label{def:nn_model}
\Phi_M(L,k, s) = \{ & \varphi(x; W, v) \in \Phi(L, d)\colon \|\varphi\|_\infty\leq M,\notag\\
&  \|W_j\|_\infty\leq 1~\text{for~}j\in[L+1],\notag\\
& \|v_j\|_\infty  \leq 1~\text{for~}j\in[L], \notag\\
&   \sum_{j = 1}^{L+1}\|W_j\|_0 + \sum_{j = 1}^L \|v_j\|_0\leq s \},
\#
where $s$ is the sparsity.  In contrast, another approach to avoid overfitting in deep learning literature is to control the norm of parameters \citep{li2018tighter}.  See Section \ref{subsection:norm_control} for details.    

Consider the following estimators via deep neural networks, 
\#\label{problem_formulation}
&\hat t(\cdot;p,q) = \argmin_{t\in\Phi_M(L,k,s)} \EE_{x\sim\PP_n}[ f^\dagger(t(x))] - \EE_{x\sim\QQ_n}[t(x)] ,\notag\\
&\hat  D_f(q\|p) =  \EE_{x\sim\QQ_n}[ \hat t(x;p,q) ] -\EE_{x\sim\PP_n}[ f^\dagger(\hat t(x;p,q) )].
\#

The following theorem characterizes the statistical rate of convergence of the estimator proposed in \eqref{problem_formulation}. 

\begin{theorem}\label{thm:main}
Let  $L = \cO(\log n)$, $s = \cO(N \log n)$, and $k = (d, d, \cO(dN), \cO(dN), \ldots, \cO(dN), 1)$ in \eqref{def:nn_model}, where $N = n^{d/(2\beta + d)}$. Under Assumptions \ref{assum:ratio}, \ref{assum:beta-holder}, and \ref{assumption:reg}, if $d < 2\beta$, then with probability at least $1- \exp\{-n^{d/(2\beta+d)}\log^5 n\}$, we have
\$
| \hat D_f(q\| p) - D_f(q\| p)| \lesssim n^{-{\beta}/{(2\beta + d)}} \log^{7/2} n. 
\$ 
\end{theorem}

\iffalse
\begin{proof}[Proof Sketch]
We consider each error bound separately. 

\noindent \textbf{Bound on $\| \hat t - t^*\|_{L_2(\PP)}$. }   By triangular inequality, we split the bound into approximation error $\|\tilde t-t^*\|_{L_2(\PP)}$ and generalization error $\|\tilde t-\hat t\|_{L_2(\PP)}$, where $\tilde t\in\Phi_M(L,k,s)$.  For the approximation error, combining the network structure, we invoke Theorem \ref{theorem:approx} to deduce that there exists some $\tilde t\in \Phi_M(L,k,s)$ such that  $\|\tilde t-t^*\|_{L_2(\PP)}\lesssim n^{-{\beta}/{(2\beta + d)}} \log^{7/2} n$, we then fix this $\tilde t$; for the generalization error, we invoke Theorem \ref{theorem:oracle_ineq}, which also concludes the result of the bound. 

\noindent\textbf{Bound on $| D_f(q\|p) - \hat D_f(q\|p) | $. }   We denote by $\cL(t) = \EE_{x\sim\QQ}[t(x)]  - \EE_{x\sim\PP}[f^\dagger(t(x))]$ and $\hat \cL(t) = \EE_{x\sim\QQ_n}[t(x)]  - \EE_{x\sim\PP_n}[f^\dagger(t(x))]$.  By triangular inequality, it holds that 
\$
| \hat D_f(q\|p) - D_f(q\|p) | = | \hat \cL(\hat t) - \cL(t^*)  | \leq | \hat \cL(t^*) - \hat \cL(\hat t) | +  | \hat \cL(t^*) - \cL(t^*) |. 
\$
For the term $| \hat \cL(t^*) - \hat \cL(\hat t) |$, by the convexity of the loss function $\hat \cL(\cdot)$, we obtain that  $| \hat \cL(t^*) - \hat \cL(\hat t) | \lesssim \| t^* - \hat t \|_{L_2(\PP)}^2$. 
Moreover, Hoeffding's inequality \citep{hoeffding1994probability} provides a bound on the term $| \hat \cL(t^*) - \cL(t^*) |$.  The above results conclude the bound on $| D_f(q\|p) - \hat D_f(q\|p) | $. 

Combining the two bounds, we finish the proof.  A detailed proof is left in Section \ref{proof:thm:main}. 
\end{proof}
\fi

We defer the proof of the theorem in Section \ref{proof:thm:main}. 
By Theorem \ref{thm:main}, the estimators in \eqref{problem_formulation} achieve the optimal nonparametric rate of convergence \citep{stone1982optimal} up to a logarithmic term.  We can see that by setting $\gamma_\Phi = d/\beta$ in Theorem \ref{thm:gen}, we recover the result in Theorem \ref{thm:main}. 
By \eqref{eq:eps2} and Theorem \ref{thm:main}, we have 
\$
&  \delta(n) = 1- \exp\{-n^{d/(2\beta+d)}\log^5 n\}, \notag\\
&  \epsilon(n) = c \cdot n^{-{\beta}/{(2\beta + d)}} \log^{7/2} n,
\$
where $c$ is a positive absolute constant. 












==> gan.tex <==
%!TEX root =pp-sample.tex

\section{Connection to $f$-GAN and Reconstruction of Distribution}\label{sec:gan}
After sample elicitation, a natural question to ask is how to learn a representative probability density function from the samples. Denote the probability density function from elicited samples as $p$. Then, learning the probability density function $p$ is to solve for
\#\label{eq:form_fgan}
q^* = \argmin_{q\in\cQ} D_{f}(q\|p),
\#
where $\cQ$ is the probability density function space.   By the non-negativity of $f$-divergence, $q^* = p$ solves  \eqref{eq:form_fgan}, which implies that by solving \eqref{eq:form_fgan}, we reconstruct the representative probability from the samples. 

To see the connection between \eqref{eq:form_fgan} and the formulation of $f$-GAN \citep{nowozin2016f}, by combining \eqref{eq:hahadf} and \eqref{eq:form_fgan}, we have
\$ %#\label{eq:popu_fgan}
q^* = \argmin_{q\in \cQ}\max_{t} \EE_{x\sim\QQ}[ t(x) ] - \EE_{x\sim\PP}[f^\dagger(t(x))],
\$ %#
which is the formulation of $f$-GAN. Here the probability density function $q$ is the generator, while the function $t$ is the discriminator. 

We now propose the following estimator, 
\#
& q^\natural = \argmin_{q\in \cQ} D_f^\natural (q\|p), \label{eq:q1-est}
\# 
where $ D_f^\natural(q\|p)$ is proposed in \eqref{eq:gen-form}. 

We impose the following assumption on the covering number of the probability density function space $\cQ$.

\begin{assumption}\label{assum:cov_num1}
We have $N_2(\delta, \cQ) = \cO( \exp\{ \delta^{-\gamma_\Phi} \})$.
\end{assumption}


The following theorem characterizes the error bound of estimating $q^*$ by $q^\natural$.
\begin{theorem}\label{theorem:outer_prob_sparsity1} 
Under the same assumptions in Theorem \ref{thm:gen}, further if Assumption \ref{assum:cov_num1} holds, for sufficiently large sample size $n$, with probability at least $1-1/n$, we have
\#\label{eq:bound-f-gan}
D_f( q^\natural \|p)  \lesssim n^{-{1}/{(\gamma_\Phi+2)}} \cdot \log n    + \min_{\tilde q\in\cQ}D_f(\tilde q\|p).
\#   
\end{theorem}



\iffalse
\begin{proof}[Proof Sketch]
We first apply union bound to the result in Theorem \ref{thm:main} for all $q$ in the space $\cQ$. In this way, we know that $\sup_{q\in \cQ}\bigl|D_f(q\|p) - \hat D_f(q\|p)\bigr| \lesssim  n^{-{2\beta}/({2\beta+d})}\cdot \log^7 n$ holds with probability at least $1-1/n$. 
Then for any $\tilde q \in \cQ$, with probability at least $1- 1/n$:
\$
D_f(\hat q\|p) & \leq \bigl|D_f(\hat q\|p) - \hat D_f(\hat q\|p)\bigr| + \hat D_f(\hat q\|p) \leq \sup_{q\in \cQ}\bigl|D_f(q\|p) - \hat D_f(q\|p)\bigr| + \hat D_f(\tilde q\|p) \\
& \lesssim n^{-{2\beta}/({2\beta+d})} \cdot \log^7 n  + D_f(\tilde q\|p). 
\$
Here in the second line we use the optimality of $\hat q$ among all $\tilde q\in \cQ$ to the problem \eqref{eq:q_outer_sample}. By taking the infimum of $\tilde q\in\cQ$ on both sides, we conclude the theorem. See Section \ref{subsection:proof_outer_prob_sparsity} for a detailed proof. 
\end{proof}
\fi

We defer the proof of Theorem \ref{theorem:outer_prob_sparsity1} in Section \ref{subsection:proof_outer_prob_sparsity1}.  In Theorem \ref{theorem:outer_prob_sparsity1}, the first term on the RHS of \eqref{eq:bound-f-gan} characterizes the generalization error of the estimator in \eqref{eq:q1-est}, while the second term is the approximation error.  If the approximation error in \eqref{eq:bound-f-gan} vanishes, then the estimator $\hat q$ converges to the true density function $q^* = p$ at the optimal nonparametric rate of convergence \citep{stone1982optimal} up to a logarithmic term. 

\begin{table*}[!ht]
%\footnotesize
\begin{small}
\centering
\begin{threeparttable}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\rule{0pt}{2ex}
\textbf{Expt.} & $\boldsymbol\mu$ & $\boldsymbol\Sigma$ & \textbf{  Analytical MI  }  & \textbf{Truthful Report} & \textbf{Random Shift}  & \textbf{Random Report} \\ \hline\hline
\rule{0pt}{4ex}
\rule[-3ex]{0pt}{0pt}
1
& $
\begin{pmatrix}
    -2.970\\ 8.977
\end{pmatrix}
$ & $
\begin{pmatrix}
    1.279 & 4.392\\ 
    4.392 & 16.187 
\end{pmatrix}
$ & 1.298 & \textbf{1.361} $\pm$ 0.062 & 1.084 $\pm$ 0.049 & 0.132 $\pm$ 0.017 \\ \cline{1-7} 
\rule{0pt}{4ex}
\rule[-3ex]{0pt}{0pt}
2 & $
\begin{pmatrix}
    6.978\\ 8.385
\end{pmatrix}
$ & $
\begin{pmatrix}
    10.545 & 16.178\\
    16.178 & 26.431 
\end{pmatrix}
$ & 1.399 & \textbf{1.322} $\pm$ 0.053 & 1.105 $\pm$ 0.044 & 0.204 $\pm$ 0.016 \\ \cline{1-7} 
\rule{0pt}{4ex}
\rule[-3ex]{0pt}{0pt}
3 & $
\begin{pmatrix}
    -3.831\\ 2.173
\end{pmatrix}
$ & $
\begin{pmatrix}
    9.545 &  9.437\\
    9.437 & 10.081
\end{pmatrix} 
$ & 1.345 & \textbf{1.462} $\pm$ 0.050 & 0.636 $\pm$ 0.041 & 0.082 $\pm$ 0.013 \\
\hline
\end{tabular}
\footnotesize{
}
\end{threeparttable}
\vspace{-3pt}
\caption{Our experiments are based on synthetic data drawn from 2-dimensional Gaussian distributions (defined by mean $\mu$ and covariance matrix $\Sigma$ in the 2nd and 3rd columns). Truthful reports lead to higher scores that are close to analytical MI.}
\label{Tab:Experiment_Results}
\end{small}
\end{table*}

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.95\textwidth]{numexpres.png}
    \vspace{-7pt}
    \caption{Convergence behavior of the three experiments. The blue solid lines refer the estimated scores and the red lines are the analytically calculated score (MI in our experiments).}
    \label{Tab:Convergence}
\end{figure*}


\subsection{Reconstruction via Deep Neural Networks}

To utilize the estimator $\hat D_f(q\|p)$ proposed via deep neural networks in Section \ref{sec:est-dnn}, we propose the following estimator, 
\#
& \hat q = \argmin_{q\in \cQ}\hat D_f(q\|p), \label{eq:q_outer_sample}
\# 
where $ \hat D_f(q\|p)$ is given in \eqref{problem_formulation}. 

We impose the following assumption on the covering number of the probability density function space $\cQ$.

\begin{assumption}\label{assum:cov_num}
We have $N_2(\delta, \cQ) = \cO( \exp\{ \delta^{-d/\beta} \})$.
\end{assumption}


The following theorem characterizes the error bound of estimating $q^*$ by $\hat q$.
\begin{theorem}\label{theorem:outer_prob_sparsity} 
Under the same assumptions in Theorem \ref{thm:main}, further if Assumption \ref{assum:cov_num} holds, for sufficiently large sample size $n$, with probability at least $1-1/n$, we have
\$
D_f(\hat q\|p) & \lesssim n^{-\frac{\beta}{2\beta+d}}\cdot \log^7 n + \min_{\tilde q\in\cQ} D_f(\tilde q\|p). 
\$
\end{theorem}

The proof of Theorem \ref{theorem:outer_prob_sparsity} is deferred in Section \ref{subsection:proof_outer_prob_sparsity2}. We can see that by setting $\gamma_\Phi = d/\beta$ in Theorem \ref{theorem:outer_prob_sparsity}, we recover the result in Theorem \ref{theorem:outer_prob_sparsity1}. 








==> num.tex <==
%!TEX root =pp-sample.tex

\section{Numerical Examples}


In order to validate our mechanism we present synthetic experiments. In the experiments, the scores are estimated based on the variational approach we documented earlier and the method used in \citep{nguyen2010estimating} for estimating the estimator. The experiments are based on synthetic data drawn from 2-dimensional Gaussian distributions \footnote{We choose simpler distribution so we can compute the scores analytically for verification purpose}. We randomly generate the means ($\mu$) and covariance matrices ($\Sigma$) for each experiment (see Table~\ref{Tab:Experiment_Results} for details.)

In general, we observe good convergence of our estimator and incentive properties in practice. Three numerical experiments are shown in Table~\ref{Tab:Experiment_Results}. In each of above experiments, we draw $1000$ pairs of samples $(x_i,y_i)$ from the corresponding Gaussian distribution. This set of pairs reflect the joint distribution $\mathbb{P}\oplus\mathbb{Q}$, while the sets $\{x_i\}$ and $\{y_i\}$ together correspond to the marginal distribution $\mathbb{P}\times\mathbb{Q}$. For each experiment, we repeat ten times and calculated the mean estimated score and the corresponding standard deviation.

For simplicity, we adopted $a=0$, $b=1$, and $f(\cdot)=-\log(\cdot)$ in estimating the scores, which make the expected score nothing but the Mutual Information (MI) between distributions $\mathbb{P}$ and $\mathbb{Q}$. The analytical values and the estimated scores of the MI for the three experiments are listed in the $4$th and $5$th column in Table~\ref{Tab:Experiment_Results}, respectively. To demonstrate the effects of untruthful reports on our score, we consider two types of untruthful reporting:
\squishlist
\item \textbf{Random Shift:} The agent draws random signals from the uniform distribution $U(0,3)$ and add them to $\{x_i\}$.
\item \textbf{Random Report;} The agent simply reports random signals that drawn from the uniform distribution $U(0,2\sigma)$, where $\sigma$ is the standard deviation of the marginal distribution $\mathbb{P}$. This models the case when agents contribute uninformative information.
\squishend

As expected, we saw the scores of untruthful reports are generally lower than the corresponding scores of truthful reports. To be complete, we also demonstrate the convergence behavior of the three experiments in Figure~\ref{Tab:Convergence}. We see that as the sample number increases the estimated scores tends to converge to their corresponding analytical values.

==> pre.tex <==
%!TEX root =pp-sample.tex



